Characterization of BNL and HPK AC-LGAD sensors with a 120 GeV proton beam

We present measurements of AC-LGADs performed at the Fermilab's test beam facility using 120 GeV protons. We studied the performance of various strip and pad AC-LGAD sensors that were produced by BNL and HPK. The measurements are performed with our upgraded test beam setup that utilizes a high precision telescope tracker, and a simultaneous readout of up to 7 channels per sensor, which allows detailed studies of signal sharing characteristics. These measurements allow us to assess the differences in designs between different manufacturers, and optimize them based on experimental performance. We then study several reconstruction algorithms to optimize position and time resolutions that utilize the signal sharing properties of each sensor. We present a world's first demonstration of silicon sensors in a test beam that simultaneously achieve better than 6-10 micron position and 30 ps time resolution. This represents a substantial improvement to the spatial resolution than would be obtained with binary readout of sensors with similar pitch.

==> oldTexFiles/ExperimentalSetup.tex <==
\section{The experimental setup at the FNAL Test Beam Facility}\label{sec:setup}

The data shown in this paper was collected at the FNAL test beam facility (FTBF)~\cite{FTBF}.
The FTBF facility supplies a \SI{120}{\GeV} proton beam as well as a silicon tracking telescope to measure the position of each incident proton.

A detailed description of the experimental setup can be found in reference~\cite{Apresyan:2020ipp}, which presents the results of a 2020 beam campaign. Since that time, several key upgrades have been made which greatly enhance the capabilities of the setup. 
These include modifications to the use of the tracking telescope, the oscilloscope used for waveform acquisition, the readout electronics, and the trigger. We describe the upgrades in this section.

In the previous setup, the silicon tracker reference resolution was degraded by the extrapolation of the proton track measured by the tracking telescope to the location of the AC-LGAD sensor at a position about \SI{2}{\m} downstream of the proton beam direction. 
The resulting resolution at the AC-LGAD sensor location was about \SI{50}{\micro \m} which rendered the measurement insensitive to the AC-LGAD position resolution. 
A new environmental chamber was constructed in order to host the AC-LGADs at the center of the telescope, as shown in Fig.~\ref{fig:FTBF_Box}. 
At this location, the position resolution of the proton track measured by the tracking telescope is in the range of 5--10\si{\micro \m}, which is comparable to the expected position resolution of the AC-LGAD sensors. 
This improvement allows extracting much more meaningful conclusions about the position resolution performance of the AC-LGAD sensors. 

The oscilloscope used in the previous campaign (Keysight MSOX92004A) provided only four readout channels, which greatly limited the ability to study the properties of multi-channel clusters. 
For this campaign, a Lecroy Waverunner 8208HD oscilloscope was acquired. 
This oscilloscope features eight readout channels with a bandwidth of \SI{2}{\giga \hertz} and a sampling rate of \SI{10}{GS/s} per channel. 
With the increased channel count, it was possible to capture fully contained clusters within the active area of the sensors, and still provide high quality waveforms for excellent spatial and time resolutions. 
The AC-LGAD under study typically used seven readout channels, while the eighth was used for the Photek micro-channel plate detector (MCP-PMT) to measure the reference time. 
The time resolution of the Photek MCP-PMT used has been measured to be about 10--15~ps. 

The AC-LGAD sensors were mounted on the readout boards optimized for LGAD sensors and capable of accommodating 16 independent channels. 
A similar version of this readout board was used in the previous measurement. 
For the current study, an upgraded version of the board was used which includes a more optimal feedback resistor to improve the signal-to-noise ratio by roughly 70\% at a small cost in signal bandwidth. 
As a result, LGAD sensors read out by the improved 16-channel board now obtain timing performance comparable to the low-noise single-channel UCSC readout board~\cite{}. 
%SX: the UCSC readout board needs a citation or further explanation
The total transimpedance on the 16-channel board after two stages of amplification is roughly \SI{4.3}{\kilo \ohm}, and no additional external amplifiers were used.

Additionally, an improved trigger was developed for this campaign, based on a \SI{3}{\milli \m} DC-LGAD sensor mounted on an independent motion stage. The trigger DC-LGAD could be aligned with the AC-LGAD under study in order to trigger only a narrow region of interest (ROI). Since the AC-LGADs are small relative to the width of the beam, the ROI trigger greatly increased the dataset purity and the acquisition rate of useful events. This improvement enabled a much larger set of sensors to be studied at a variety of operating conditions within the limited period of available beam time.

% \begin{itemize}
%     \item Location of the box within the telescope. Resolution improvement of \SI{50}{\micro \m} to \SI{12}{\micro \m}
%     \item Increased number of readout channels. From 3 to 7.
%     \item Improved trigger efficiency. Went from using a scintillator to a large LGAD as the source of the trigger
%     \item Improved design of readout board. Better S/N with new \SI{50}{\ohm} feedback resistor
% \end{itemize}

\begin{figure}[ht!]
\centering
\includegraphics[width=0.99\textwidth]{pictures/TestBeamPic.jpg}
\caption[FTBF Box]{A photograph of the environmental chamber placed within the FTBF silicon telescope
\label{fig:FTBF_Box}}
\end{figure}


Since the position resolution of the tracker telescope measurement at the AC-LGAD location is now comparable to the expected resolution of the AC-LGAD sensors, the calibration of the tracker telescope is extremely important. 
Several methods were used to estimate the tracker spatial resolution. 
First, the track reconstruction algorithm based on the Kalman filter provides an estimate of the impact parameter resolution for each track based on the compatibility of the track fit with the observed hits. 
This yields an estimated resolution of roughly \SI{5}{\micro \m}. 
Second, the resolution was estimated by studying the smearing of the efficiency turn-on curve at the edge of a DC-LGAD sensor. 
Assuming the true LGAD efficiency curve is a perfect step function on the micron scale, then any observed smearing can be attributed to the tracker resolution and extracted by a fit to an error function model. 
Finally, the resolution was also estimated using strip sensors with known pitch using binary readout.
In a binary readout scheme, the resolution is simply the pitch divided by $\sqrt{12}$. 
Any enhancement of the resolution beyond this value is attributed as the tracker impact parameter resolution. 
In both the DC-LGAD edge fit and the binary readout methods, the resolution obtained is in the range of \SIrange{10}{12}{\micro \m}, somewhat at tension with the \SI{5}{\micro \m} result obtained from the Kalman filter. 
Since the Kalman filter resolution does not include contributions from the alignment with the device under test, we take its estimate as a lower bound. 
Conversely, since the two other methods may contain additional systematic errors, we take their estimates as upper bounds on the resolution. 
As result, we limit the tracker resolution to a range of roughly 5--10 \si{\micro \m} and use this range to interpret the observed AC-LGAD performance.

==> oldTexFiles/HPK_results.tex <==
\subsection{HPK Results}

{\color{blue} {Will: I created this new subsection and put ten HPK figures in it. I had to convert five of them from .gif to .pdf because Overleaf did not recognize the format. 

We should discuss whether we want the form 1)BNL sensor section, followed by 2)HPK sensor section, or something more intermingled.

We should go through the plots to discuss which ones should appear in the paper and which ones to omit. Once that's decided I can start writing text about the ones that are kept. All of the figures are piling up at the end due to lack of text to balance them.}}

\begin{figure}
    \centering
    \begin{subfigure}{0.4\textwidth}
        \includegraphics[width=\textwidth]{plots/HPK_pads_C2/TotalAmplitude_vs_x.pdf}
        \caption{HPK C2 pad}
        \label{fig:TotalAmp_HPKC2p}
    \end{subfigure}
    \begin{subfigure}{0.4\textwidth}
        \includegraphics[width=\textwidth]{plots/HPK_pads_B2/TotalAmplitude_vs_x.pdf}
        \caption{HPK B2 pad}
        \label{fig:TotalAmp_HPKB2p}
    \end{subfigure}
    \caption{Most Probable Value of the total amplitude over the sensor and per pad vs position, using the nominal voltage.}
    \label{fig:TotalAmp_HPKp}
\end{figure}

\begin{figure}
    \centering
    \begin{subfigure}{0.4\textwidth}
        \includegraphics[width=\textwidth]{plots/HPK_pads_C2/PositionFitTop.pdf}
        \caption{HPK C2 pad}
        \label{fig:PositionFit_HPKC2p}
    \end{subfigure}
    \begin{subfigure}{0.4\textwidth}
        \includegraphics[width=\textwidth]{plots/HPK_pads_B2/PositionFitTop.pdf}
        \caption{HPK B2 pad}
        \label{fig:PositionFit_HPKB2p}
    \end{subfigure}
    \caption{Fit to the amplitude distribution in the upper left pad over the upper half of the sensor, using the nominal voltage.}
    \label{fig:PositionFit_HPKp}
\end{figure}

\begin{figure}
    \centering
    \begin{subfigure}{0.4\textwidth}
        \centering
        \includegraphics[width=\textwidth]{plots/HPK_pads_C2/PositionRes_vs_x_track.pdf}
        \caption{HPK C2 pad}
        \label{fig:PositionRes_HPKC2p}
    \end{subfigure}
    \begin{subfigure}{0.4\textwidth}
        \centering
        \includegraphics[width=\textwidth]{plots/HPK_pads_B2/PositionRes_vs_x_track.pdf}
        \caption{HPK B2 pad}
        \label{fig:PositionRes_HPKB2p}
    \end{subfigure}
    \caption{Position resolution of the pad detectors vs tracker relative position, for nominal voltages. Only the inner half of the detector is studied, demarcated by the red lines, to avoid edge effects.}
    \label{fig:PositionRes_HPKp}
\end{figure}

\begin{figure}
    \centering
    \begin{subfigure}{0.4\textwidth}
        \centering
        \includegraphics[width=\textwidth]{plots/HPK_pads_C2/TimeRes_vs_x_weighted2_time_diff.pdf}
        \caption{HPK C2 pad}
        \label{fig:TimeRes_HPKC2p}
    \end{subfigure}
    \begin{subfigure}{0.4\textwidth}
        \centering
        \includegraphics[width=\textwidth]{plots/HPK_pads_B2/TimeRes_vs_x_weighted2_time_diff.pdf}
        \caption{HPK B2 pad}
        \label{fig:TimeRes_HPKB2p}
    \end{subfigure}
    \caption{Time resolution of the pad detectors vs tracker relative position, for nominal voltages. Only the inner half of the detector is studied, demarcated by the red lines, to avoid edge effects.}
    \label{fig:TimeRes_HPKp}
\end{figure}

\begin{figure}
    \centering
    \begin{subfigure}{0.4\textwidth}
        \centering
        \includegraphics[width=\textwidth]{plots/HPK_strips_C2/45um_Amp_inStrip0_fromHit_inOtherChs.pdf}
        \caption{HPK C2 45 $\mu$m strip}
        \label{fig:AmpChSh_HPK45s}
    \end{subfigure}
    \begin{subfigure}{0.4\textwidth}
        \centering
        \includegraphics[width=\textwidth]{plots/HPK_strips_C2/30um_Amp_inStrip0_fromHit_inOtherChs.pdf}
        \caption{HPK C2 30 $\mu$m strip}
        \label{fig:AmpChSh_HPK30s}
    \end{subfigure}
    \caption{Signal recorded in the first (0th) strip when the actual hit occurred in the same (solid line) or in another (dashed line) strip. The presence of a peak coming from hits in the opposite channel shows that the effects of Charge Sharing impact greatly the performance of the detection.}
    %\caption{Charge Sharing effect recorded in the first (0th) strip when the actual hit occurred in the same (solid line) or in another (dashed line) strip.}
    \label{fig:AmpChSh_HPKs}
\end{figure}

%\begin{figure}
%    \centering
%    \includegraphics[width=10cm]{plots/HPK_strips_C2/45um_Amp_inStrip0_fromHit_inOtherChs.pdf}
%    \caption{Charge Sharing effect recorded in the first (0th) strip when the actual hit occurred in the same (solid line) or in another (dashed line) strip, for HPK C2 45 $\mu$m strip detector.}
%    \label{fig:AmpChSh_HPKC2s}
%\end{figure}



==> oldTexFiles/PositionReco.tex <==
\subsection{Position reconstruction}
The resolution of the hit position reconstruction can be significantly improved by utilizing the charge sharing property in AC-LGAD sensors. 
To achieve the improved position resolution, we interpolate the position between two strips using the signal size information from multiple neighboring strips.
We present two different methods for achieving this interpolation. 
The first method is a simple approach where we determine the interpolated position based on the amplitude ratio of the strip with the maximal signal and its neighboring strips. 
The second method uses a machine learning technique by feeding the measured amplitudes of all channels to a neural network trained to target the measured position from the tracking telescope.
The measurement of the position resolution will be limited by the position resolution of the tracks reconstructed by the tracking telescope.

\subsubsection{Amplitude ratio method}
In the simple method, we use the amplitudes for the leading and sub-leading channels for the position interpolation.
For the strip sensors, the sub-leading channel may be on the left or right side of the maximum amplitude channel, and only the x coordinate of the hit position is obtained.
For the large pad sensors we used the channel corresponding to the horizontal (vertical) neighbor of the maximum amplitude channel for the x (y) coordinate of the hit position.
For each sensor, the average position coordinate measured by the tracking telescope is plotted against the average amplitude fraction $a_1/(a_1+a_2)$, where $a_1$ and $a_2$ are the amplitudes of the maximum amplitude and sub-leading channels, and then fitted to a $3^{\rm{rd}}$--$5^{\rm{th}}$ degree polynomial to obtain a model for the relationship between amplitude fraction and hit position coordinate. 
The model was obtained using the nominal voltages for each sensor, though it was observed that the relationship was independent of the bias voltage.

The fit function model for the BNL 2020 strip sensor is shown on the left of Figure~\ref{fig:posFitBNL2020}, while on the right we show the position resolution as a function of the hit position measured by the tracking telescope.
We call this method of the reconstructing the charge particle hit position the "two--strip" position reconstruction.
Both plots in Figure~\ref{fig:posFitBNL2020} show the location of the metallic region for each strip in the sensor.
The model to map the amplitude ratio onto the reconstructed position is only defined for the region between the center of the maximum amplitude strip to the center of the gap between the max amplitude and sub-leading amplitude strips.
The absolute position is obtained by adding the position obtained from the fit function model on the left of Figure~\ref{fig:posFitBNL2020} to the position of the center of the maximum amplitude strip.
We measure a position resolution of about 5~$\mu$m using the two-strip method, which improves by about a factor of 6 over the simplest method of taking the center of the maximum amplitude strip, corresponding to a resolution of $\rm{pitch}/\sqrt{12}$.

\begin{figure}[htp]
    \centering
    \includegraphics[width=0.49\textwidth]{plots/BNL2020/PositionFit.pdf}
    %\includegraphics[width=0.49\textwidth]{plots/PositionRes_vs_x_deltaXmax_vs_xreco_BNL2020}
    \includegraphics[width=0.49\textwidth]{plots/BNL2020/PositionRes_vs_x_track.pdf}
    \caption[Amp BNL 2020]{%\textcolor{red}{RH, right legend: "Binary readout","Two-strip reconstruction"}
    Fit of the amplitude ratio as a function of tracker position from center of strips on BNL 2020 sensor (left). Position resolution as a function of tracker position (right). \textcolor{red}{exactly 50 micron bins, offset by 0.5 bin. Center of bin will alternating coinciding with center of strip OR center of gaps. Larger font size. Move legend down and stop y-axis around 35 microns. axis: Track x position [mm]. Left plot: Amplitude fraction in leading strip.} 
    \label{fig:posFitBNL2020}}
\end{figure}

The fit function model and the measured position resolution for the HPK C2 large pad array sensor is shown in Figure~\ref{fig:PositionFit_HPKC2p}.
Because the pad sensors are in a 2x2 array configuration, the fit function directly models the absolute hit position on the sensor rather than the offset from the center of the maximum amplitude strip.
For the x coordinate measurement, we show the measurement using the top left and top right sensors. Consistent results were observed for the bottom row using the bottom left and bottom right sensors.
The y coordinate measurement shown is done using the top left and bottom left sensors. Similarly, the measurements using the top right and bottom right sensors yielded consistent results.
%SX: i also do not see a y-position plot at all. should we put that in? could be done as a 2nd graph/hist in the right of FIg10 and relabel axis as x/y position. 
The utilization of charge sharing for these large 500$x$\SI{500}{\micro\metre} pitch sensors improves the position resolution by a factor of about 7 from \SI{144}{\micro\metre} using the center of the maximum amplitude channel to about \SI{20}{\micro\metre} using the amplitude ratio method as shown in Figure~\ref{fig:PositionFit_HPKC2p}.
Unlike the strip sensors shown in Figure~\ref{fig:posFitBNL2020} the position resolution for the large pad sensors is not uniform and reaches a best value in the center between two channels. 
This is a consequence of the amplitude ratio becoming flat as a function of position for charged particle hits near the center of the pads.

\begin{figure}[htp]
    \centering
    \includegraphics[width=0.49\textwidth]{plots/HPK_pads_C2/PositionFitTop.pdf}
    \includegraphics[width=0.49\textwidth]{plots/HPK_pads_C2/PositionRes_vs_x_track.pdf}
    \caption[Amp HPK C2]{Fit of the amplitude distribution in the upper left pad over the upper half of the HPK C2 pad sensor, using the nominal voltage (left). Position resolution as a function of tracker position (right).
    \textcolor{red}{Amplitude fraction in right pad. Fewer bins and line up better with red lines}
    \label{fig:PositionFit_HPKC2p}}
\end{figure}

%\begin{figure}
%    \centering
%    \begin{subfigure}{0.4\textwidth}
%        \includegraphics[width=\textwidth]{plots/HPK_pads_C2/PositionFitTop.pdf}
%        \caption{HPK C2 pad}
%        \label{fig:PositionFit_HPKC2p}
%    \end{subfigure}
%    \begin{subfigure}{0.4\textwidth}
%        \includegraphics[width=\textwidth]{plots/HPK_pads_B2/PositionFitTop.pdf}
%        \caption{HPK B2 pad}
%        \label{fig:PositionFit_HPKB2p}
%    \end{subfigure}
%    \caption{Fit to the amplitude distribution in the upper left pad over the upper half of the sensor, using the nominal voltage.}
%    \label{fig:PositionFit_HPKp}
%\end{figure}

%\begin{figure}
%    \centering
%    \begin{subfigure}{0.4\textwidth}
%        \centering
%        \includegraphics[width=\textwidth]{plots/HPK_pads_C2/PositionRes_vs_x_track.pdf}
%        \caption{HPK C2 pad}
%        \label{fig:PositionRes_HPKC2p}
%    \end{subfigure}
%    \begin{subfigure}{0.4\textwidth}
%        \centering
%        \includegraphics[width=\textwidth]{plots/HPK_pads_B2/PositionRes_vs_x_track.pdf}
%        \caption{HPK B2 pad}
%        \label{fig:PositionRes_HPKB2p}
%    \end{subfigure}
%    \caption{Position resolution of the pad detectors vs tracker relative position, for nominal voltages. Only the inner half of the detector is studied, demarcated by the red lines, to avoid edge effects.}
%    \label{fig:PositionRes_HPKp}
%\end{figure}

\subsubsection{Machine learning analysis}
As an alternative position reconstruction algorithm, a neural network (NN) based regression was trained to reconstruct particle hit location within the sensor.
As a general motivation, there are situations in which the NN could outperform the reconstruction method described previously in terms of latency due to the fact that it is based on linear operations that are faster to evaluate on certain FPGAs and ASIC chips.
The functional form used for the amplitude ratio fits could become non-linear which are not ideal for front-end electronics. 

The NN was trained on data collected with the BNL 2020 sensor and used the position from the FNAL tracking telescope as a target for the reconstructed position. 
The selection of the data is identical to the selection used for the analysis described previously.
The NN was trained using a Keras-based~\cite{chollet2015keras} code framework.
The data was randomly split into three categories: training, testing, and validation. 
The training, testing, and validation categories are comprised of 80\%, 10\%, and 10\% of the total data, respectively.

The input variables for the NN is the measured amplitudes and time from each channel in the sensor.
%The NN model is a fully connected dense NN (DNN) with three hidden layers and can be seen in Figure~\ref{fig:NNModel}.
The NN model is a fully connected dense NN (DNN) with three hidden layers.
The input layer is passed to a lambda layer that transforms each of the inputs such that their respective distributions have a mean of zero and standard deviation of one.
The number of nodes for each hidden layers was set to one hundred and the activation function for each of the hidden layers was set to the commonly used rectified linear unit (ReLU) function.
The output layer has only one value for its output and does not use an activation function.
The model is then trained using the Adam optimizer and by using the mean squared error as the loss function. 
%SX: do we need a citation for Adam optimizer? What is that?
The model is supervised to predict the position measured by the FNAL tracking telescope.
All hyper--parameters are scanned to determine the optimal values for each one.

%\begin{figure}[htp]
%\centering
%\includegraphics[width=0.49\textwidth]{plots/model_NN}
%\caption[NN model]{Diagram of the NN model made using the Keras software.
%\label{fig:NNModel}}
%\end{figure}

The final results are compared to the telescope position to measure the position resolution from the NN method.
The performance is almost identical compared to the results obtained with the simplified method shown above.
Because the NN is trained to target the tracking telescope measurements, the position resolution will be limited by the resolution of the telescope. 
%SX: I think we should motivate this ML reconstruction method a bit further by talking about the possibility to apply these NN on readout chips or readout FPGAs. There are situations in which the NN could outperform the "simpler" method in terms of latency due to the fact that it is based on linear operations that are faster to evaluate on certain FPGAs and ASIC chips. The simpler methods may potentially rely on evaluating non-linear functions which may be ok on CPUs but maybe is not that great on chips. In our specific case I think it doesn't really...but I think for the reader we should set up some motivations that is giving a clear reason of why you would ever use NN method over the simpler method. Otherwise, the reader or reviewer would ask why are you even studying the NN thing at all. 
Therefore, the overall performance difference between the two reconstruction approaches can not be discerned at this stage.

%\begin{figure}[htp]
%\centering
%\includegraphics[width=0.49\textwidth]{plots/xResROOT_NN_BNL2020}
%\caption[NN Result]{Comparison of the NN output to the FNAL telescope value.
%\label{fig:NNResults}}
%\end{figure}


==> oldTexFiles/SensorBackground.tex <==
\section{The AC-LGAD sensor}\label{sec:sensor}

%SX: We should have a general intro paragraph to tell the reader what an LGAD is, and what an AC-LGAD is? 
We studied four different AC-LGAD sensors, designed and produced by BNL and KEK/Tsukuba.

The first two sensors under study were fabricated at BNL, see Fig.~\ref{fig:BNL2020Pic}, using a class-100 silicon processing facility and following the process outlined in reference~\cite{ACLGADprocess}.
The sensors comes from two different wafers which underwent a very similar process in the clean room.
The wafers are 4-inches p-type epitaxial wafers, where the 50~$\mu$m-thick epitaxial layer has been grown over a 0.5~mm thick low-resistivity substrate. 
The epitaxial layer has a depletion voltage of 120~V with $N_C = 7 \cdot 10^{13}$~$\mathrm{cm}^{-3}$.
%SX: shouldn't we define what N_C means?

The first AC-LGAD sensor, shown on the left panel of Fig.~\ref{fig:BNL2020Pic}, has an active area of about $2\times2$~mm${}^2$, and consists of an array of 17 AC-coupled metal strips surrounded by a DC-connected pad. 
The sensors are 100~$\mu$m in pitch consisting of 1.7~mm long metallized pads which are 80~$\mu$m wide with an inter-strip gap of 20~$\mu$m. 
%The strips are about 1.7~mm long and have a pitch of 100~$\mu$m consisting of a metallized width of 80~$\mu$m and an inter-strip gap of 20~$\mu$m. 
This sensor has been used in a previous study~\cite{Apresyan:2020ipp}, where more details of its cross section and parameters are described.
The second AC-LGAD sensor, shown on the right panel of Fig.~\ref{fig:BNL2020Pic}, has been cut from a different wafer. 
It has an active area of $3\times3$~mm${}^2$ and consists of three different arrays each with 6 AC-strips that are 80~$\mu$m wide. 
The three arrays have pitch of 100, 150 and 200 $\mu$m with a strip length of about 2.5~mm, varying slightly between the three arrays to keep the distance from the grounded metal of the DC-contact as large as their gap with neighbouring strips.
The two sensors have the same thickness of the dielectric composed of about 100 nm of PECVD silicon nitride, the same dose of $n^+$ implant of about 100 times less than in a standard DC-LGAD, the same breakdown voltage of about 200V, and the same geometry of the termination.

The third and fourth AC-LGAD prototype sensors were developed by KEK/Tsukuba using the Hamamatsu HPK layout~\cite{HPKsensorRef}. 
The first of these, shown on the left of Fig.~\ref{fig:HPK2020Pic}, has four pad electrodes of size $500\times500$~$\mu$m${}^2$. 
The second HPK device, shown on the right of Fig.~\ref{fig:HPK2020Pic}, features $9.88$~mm long strip electrodes with an $80$~$\mu$m pitch. 
Both devices have an active thickness of 50~$\mu$m. 
A variety of n+ and p+ doping concentrations, ranging from A through E and 1 through 3, were studied in test samples to optimize signal size and minimize crosstalk; the pad device discussed here was fabricated with C-2 and B-2, while the strip device was fabricated with C-2 type.
%SX: we need to give more information about the A-E and 1-3 doping concentration variations. What are the numerical values of these concentrations? do we know those numbers and are we allowed to give those numbers here? If not, then we need to change the sentence here to be more vague and not specifically point to B-2 and C-2 because otherwise the reader will not understand what those labels mean. 
The strips have a narrow aluminum metallization to reduce capacitance, and relatively high n+ implant resistivity. The pads have relatively low n+ resistivity with the aim of using charge sharing to achieve improved spatial resolution using high-resolution readout digitization. The aluminum strips were deposited in widths of 30,~35,~40,~and~45~$\mu$m, allowing systematic studies of the impact of varying that parameter.

{\color{violet} {Claudio: idk if this should be here, in the 'Experimental Setup' section or later, but it would be great to explain that HPK sensors have a nominal voltage of: 180 [V] (HPK C2 pad), 230 [V] (HPK B2 pad) and 170 [V] (HPK strips); and that some measurements were made altering the bias voltage for the pads (to check effects), but for strips we only have the nominal value.}}

\begin{figure}[htp]
\centering
\includegraphics[width=0.32\textwidth]{pictures/BNL2020_pic.png}
\includegraphics[width=0.32\textwidth]{pictures/BNL2021_pic.png}
%\includegraphics[width=0.32\textwidth]{plots/HPK_pic}
\caption[Sensor picture]{The BNL manufactured sensors tested at FNAL. BNL 2020 sensor (left) with 100~$\mu$m pitch and 20~$\mu$m gap sizes. BNL 2021 sensor (right) with three pitch variation 100~$\mu$m (narrow), 150~$\mu$m (medium), 200~$\mu$m (wide).}
\label{fig:BNL2020Pic}
\end{figure}

\begin{figure}[htp]
\centering
\includegraphics[width=0.32\textwidth]{pictures/HPKpad.jpg}
\includegraphics[width=0.45\textwidth]{pictures/HPKstrip.jpg}
\caption[Sensor picture]{The KEK/Tsukuba HPK sensors tested at FNAL. The four-pad device (left) with each pad being $500\times500\mu$m${}^2$ in size. Despite the relatively large area, quite precise position information can be obtained through the use of charge sharing information in the analysis. The narrow strip device (right). The centers of the aluminum metallization regions are separated by a strip pitch of 80~$\mu$m. The width of the aluminum deposited varied from 30 to 45 $\mu$m, in 5 $\mu$m steps.}
\label{fig:HPK2020Pic}
\end{figure}

==> oldTexFiles/Signal_Properties.tex <==
\subsection{Signal properties}
%cluster size plot: profile plot, talk about edge effects and stress bulk vs. edge effects. Overlay all sensor on one plot?  Use common threshold for this plot only. 
%Amplitude threshold that correspond to ~5 fC signal? 

After defining an appropriate event selection, we study the signal properties beginning with the size of the signal amplitudes in the channel closest to the proton hit as well as the neighboring channels. Subsequently we combine information from multiple channels to reconstruct the position and time of each charged particle hit. 

The mean signal amplitude size is a parameter critical to the expected performance of the sensor.
We rank the amplitude sizes among each of the strips that are read out per event and plot the ranked amplitudes in Fig.~\ref{fig:AmpChSh_HPKs} for the BNL and HPK strip sensors. Due to the charge sharing properties of the AC-LGAD sensors we observe signals with amplitude well above noise for channels that did not have a direct impact from the charge particle. The size of the signal amplitude decreases for strips that are increasingly further away from the strip with the maximum amplitude signal. 

%\begin{figure}[htp]
%\centering
%\includegraphics[width=0.47\textwidth]{plots/BNL2020/ampRankPlot.pdf}
%\includegraphics[width=0.47\textwidth]{plots/BNL2021/ampOverCh2.pdf}
%\includegraphics[width=0.50\textwidth]{plots/BNL2020/TotalAmplitude_vs_x_BNL2020%}
%\caption{Plot of the measured amplitude from each stripped ranked by the amplitude for any given event. Each curve is normalized to unit area. The amplitude ranking for BNL 2020 sensor (left). The amplitude ranking for BNL 2021 medium pitch senor (right). \textcolor{red}{Extend x-axis for 2021 frame. Combine with figure 6: left side will be 2021 BNL, right side will be 45 micron HPK. Add header, increase font size. Axis label "Signal amplitude"} \textcolor{violet}{Done! Updated in the next figure.}}
%\label{fig:ampRankBNLStrips}
%\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.49\textwidth]{plots/BNL2021/ampOverCh2.pdf}
    %\caption{HPK C2 45 $\mu$m strip}
    %\label{fig:AmpChSh_HPK45s}
    \includegraphics[width=0.49\textwidth]{plots/HPK_strips_C2/ampOverCh2.pdf}
    %\caption{HPK C2 30 $\mu$m strip}
    %\label{fig:AmpChSh_HPK30s}
    \caption{Signal recorded in the third strip when the actual hit occurred in the same (solid line) or in another (dashed line) strip.
    Each curve is normalized to unit area. The amplitude ranking for BNL 2021 medium pitch senor (left).
    } %The presence of a peak coming from hits in the opposite channel shows that the effects of Charge Sharing impact greatly the performance of the detection.}
    %\caption{Charge Sharing effect recorded in the first (0th) strip when the actual hit occurred in the same (solid line) or in another (dashed line) strip.}
    \label{fig:AmpChSh_HPKs}
\end{figure}


In each bin of the proton hit position in the direction perpendicular to the strip orientation (x), we fit the signal amplitude histogram to the convolution of a Landau distribution and a Gaussian function to model the charge deposit of a minimum ionizing particle. We extract the $\mu$ or most probable value (MPV) parameter of the Landau distribution to characterize the size of the signal observed in each strip.  Figures~\ref{fig:ampVsXBNL}~and~\ref{fig:TotalAmp_HPKp} show the MPV as a function of the x coordinate of the proton hit position for each channel individually as well as the sum for all channels for the BNL and HPK sensors, respectively. The shaded gray regions indicate the metallic regions for each sensor.

\begin{figure}[htp]
\centering
%\includegraphics[width=0.47\textwidth]{plots/BNL2021/ampRankPlot_BNL2021medium}
\includegraphics[width=0.49\textwidth]{plots/BNL2020/TotalAmplitude_vs_x.pdf}
\includegraphics[width=0.49\textwidth]{plots/BNL2021/TotalAmplitude_vs_x_medium.pdf}
\caption[Amp BNL 2021 medium]{MPV value for Landau functional fits to amplitude distributions as a function of tracker position. Each plot shows the MPV amplitude value for each strip individually as well as the total sum of each strip. Amaptude MP as a function of tracker position for the BNL 2020 (left) and BNL 2021 medium pitch (right) sensors. \textcolor{red}{Drop total histogram. Make y-axis range the same for both frames. x-axis title: "Track x position [mm]"
\textcolor{violet}{Done! Font size have to be improved (Check which one fits better).}} 
\label{fig:ampVsXBNL}}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.49\textwidth]{plots/HPK_pads_C2/TotalAmplitude_vs_x.pdf}
    %\caption{HPK C2 pad}
    %\label{fig:TotalAmp_HPKC2p}
    \includegraphics[width=0.49\textwidth]{plots/HPK_pads_B2/TotalAmplitude_vs_x.pdf}
    %\caption{HPK B2 pad}
    %\label{fig:TotalAmp_HPKB2p}
    \caption{Most probable value of the total amplitude over the sensor and per pad vs position, using the nominal voltage.
    \textcolor{red}{Drop total histogram. Make y-axis range the same for both frames. Zoom x-axis to minimize white space}
    \textcolor{violet}{Done! Maybe the font size have to be improved.}}
    \label{fig:TotalAmp_HPKp}
\end{figure}

%\begin{figure}[htp]
%\centering
%\includegraphics[width=0.47\textwidth]{plots/BNL2021/ampRankPlot_BNL2021narrow}
%\includegraphics[width=0.50\textwidth]{plots/BNL2021/TotalAmplitude_vs_x_BNL2021narrow}
%\caption[Amp BNL 2021 narrow]{BNL 2021 Narrow
%\label{fig:ampBNL2021Narrow}}
%\end{figure}


%\begin{figure}[htp]
%\centering
%\includegraphics[width=0.47\textwidth]{plots/HPK/TotalAmplitude_vs_x_HPKC2.gif}
%\includegraphics[width=0.50\textwidth]{plots/HPK/TotalAmplitude_vs_Y_HPKC2.gif}
%\caption[Amp HPK C2]{HPK C2
%\label{fig:ampHPKC2}}
%\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%To study the effects of charge sharing more closely, we define the cluster size to be the number of channels with signal charge above the noise threshold of 10~fC near each proton hit.
%In Fig.~\ref{fig:clusterVsX} we show the average cluster size for the BNL 2020 and BNL 2021 medium pitch strip sensors as a function of the x position of the proton hit. We observe that the average cluster size increases smoothly from one to two as the charged particle hit moves from the center of a strip to the gap between two neighboring strips. The average cluster size for all of the other sensors studied are summarized in Table~\ref{table:SignalProp}.

%\begin{figure}[htp]
%\centering
%\includegraphics[width=0.49\textwidth]{plots/BNL2020/Cluster_vs_x_BNL2020}
%\includegraphics[width=0.49\textwidth]{plots/BNL2021/Cluster_vs_x_BNL2021medium}
%\caption[Eff BNL 2020]{Average cluster size of the BNL 2020 (left) and BNL 2021 medium pitch (right) sensors as a function of the x coordinate of the proton hit position. Cluster size is defined as the number of strip channels with signal charge larger than 10~fC. 
%\label{fig:clusterVsX}}
%\end{figure}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
We also measure the MIP detection efficiency of each sensor, defined as the number of events passing the amplitude requirement discussed in Section~\ref{sec:results} divided by the number of events for which a track was reconstructed and whose hit position is within the active region of the sensor. 
We observed that all sensors were fully efficient across their surfaces.
Fig.~\ref{fig:effBNLStrip} shows the MIP detection efficiency of each strip of the BNL sensors as well as the efficiency for any strip to detect a signal passing the amplitude requirement. With the charge sharing properties of the BNL sensors, the MIP detection efficiency can be maintained at 100\% also in the gaps between pairs of strips.

\begin{figure}[htp]
\centering
\includegraphics[width=0.49\textwidth]{plots/BNL2020/Efficiency_HighThreshold_vs_x.pdf}
\includegraphics[width=0.49\textwidth]{plots/BNL2021/Efficiency_HighThreshold_vs_x_medium.pdf}

%\includegraphics[width=0.49\textwidth]{plots/BNL2021/Efficiency_HighThreshold_vs_x_BNL2021_narrow}
%\includegraphics[width=0.49\textwidth]{plots/BNL2021/Efficiency_HighThreshold_vs_x_BNL2021_wide}
\caption[Eff BNL 2020]{Responds efficiency of the BNL 2020 (left) and BNL 2021 medium (right) sensors. 
\label{fig:effBNLStrip}}
\end{figure}


%\begin{itemize}
%    \item how large are the signals
%    \item cluster properties: how far is the charge sharing, what's the number of clusters, number of strips per cluster, 
%    \item uniformity of sensors
%    \item comparison/discussion of different sensors
%\end{itemize}

%\begin{figure}[htp]
%\centering
%\includegraphics[width=0.49\textwidth]{plots/BNL2020/clusterSize_BNL2020}
%
%\includegraphics[width=0.32\textwidth]{plots/BNL2021/clusterSize_BNL2021wide}
%\includegraphics[width=0.32\textwidth]{plots/BNL2021/clusterSize_BNL2021medium}
%\includegraphics[width=0.32\textwidth]{plots/BNL2021/clusterSize_BNL2021narrow}
%\caption[Eff BNL 2020]{Cluster BNL2020 top and BNL2021 bottom wide, medium, narrow 10 fC. Most likely will move info to a table
%\label{fig:cluster1D}}
%\end{figure}

\begin{table}[htp]
  \centering
  \caption{Summary of each sensor's signal properties \textcolor{red}{discuss differences in sensors in text, subtracted 5 and 7 micron for position res. can't do 9 or 10 since we measure 8 for some sensors}}
  \begin{tabular}{| l | c | c | c | c | c | c |}
  \hline
  Name            & Pitch & MPV Amp. [mV] & Position Res. [$\mu$m] & Time Res. [ps]\\  
  \hline 
  BNL 2020          & 100   & 101   & [5.0--7.0]     & 26.2     \\ \hline
  BNL 2021 Narrow   & 100   & 104   & [6.5--8.1]     & 37.0     \\
  BNL 2021 Medium   & 150   & 136   & [10.5--11.6]   & 24.8     \\
  BNL 2021 Wide     & 200   & 144   & [8.4--9.7]     & 33.3     \\ \hline
  HPK C--2          & 500   & 128   & [18.8--19.4]    & 25.2     \\ \hline
  HPK B--2          & 500   & 95    & [24.0--24.5]    & 21.5     \\
  \hline
  \end{tabular}
  \label{table:SignalProp}
\end{table}

%& Cluster size & Noise [mV] 
%& 1.492        & 2.063      
%& 1.588        & 3.311      
%& 1.582        & 2.193      
%& 1.508        & 2.566      
%& -            & 2.196      
%& -            & 2.147      

%SX: Table above needs to say that the amplitude column is the amplitude of the maximum channel
%SX: we need to discuss numbers of the table above. Discuss that signal size depends on pitch size, and geometry. 

%% RH: remove noise, cluster. Revisit time resolution. Position: subtrack 5 or 9 and quote range



==> oldTexFiles/TimeReco.tex <==
\subsection{Time reconstruction}
Similar to position reconstruction, charge sharing can also be utilized to improve the time measurement of the AC-LGAD sensor.
The simplest approach for reconstructing the time for a given particle hit is to use the time measured for the channel with the largest signal amplitude.
However this approach leads to non-uniform time resolution across the sensor because the resolution becomes worse in the gaps between strips.
This is due to reduced signal to noise ratio in the largest amplitude channel because significant fraction of the signal is instead recorded by a neighboring strip.
An improved method calculates timestamps according to the amplitude-weighted average of multiple channels as follows
\begin{equation}
    t_{\rm{reco}} = \frac{\sum_{i}{a_i^2t_i}}{\sum_{i}{a_i^2}},
\label{eq:recotime}
\end{equation}
where $a_{i}$ and $t_{i}$ are the amplitude and time measurements of strip $i$.
Using this time reconstruction method leads to an improvement in the time resolution of the sensor in the gaps between the strips.

We show measurements of the time resolution for the BNL2020 sensor as a function of the hit position along the axis perpendicular to the strip orientation in Fig.~\ref{fig:timeResvsX}. The time resolution is measured with respect to the time measurement from the Photek MCP-PMT. The time resolution of the Photek MCP-PMT has been measured to be about 10~ps and is subtracted from time resolution measurements shown. On the left of Fig.~\ref{fig:timeResvsX} we show the time resolution using the simple method that uses the timestamp only from the highest amplitude strip. We observe the resolution becoming noticeably worse when the particles are impacting near the gap between adjacent strips. On the right of Fig.~\ref{fig:timeResvsX} we show the time resolution using the amplitude-weighted average, and we observe a clear improvement in the time resolution close to the gaps and a much more uniform behavior across the entire sensor. The time resolution for the BNL sensor is about 30~ps. 


\begin{figure}[htp]
\centering
\includegraphics[width=0.49\textwidth]{plots/BNL2020/TimeRes_vs_x_BothMethods.pdf}
\includegraphics[width=0.49\textwidth]{plots/HPK_pads_C2/TimeRes_vs_x_BothMethods.pdf}
%\includegraphics[width=0.49\textwidth]{plots/HPK_pads_C2/TimeRes_vs_x_BothMethods_160V.pdf}
\caption[Amp BNL 2020]{Time resolution as a function of tracker position relative to the center with different methods, for the BNL 2020 sensor (left) and HPK C2 pad with a Bias Voltage of 160 [V] (right).
\label{fig:timeResvsX}}
%  Reconstruction time coming from the time of the max amplitude strip (left). Reconstruction time coming from the squared amplitude weighted time of all non-noisy strips (right).
\end{figure}

%\begin{figure}
%    \centering
%    \begin{subfigure}{0.4\textwidth}
%        \centering
%        \includegraphics[width=\textwidth]{plots/HPK_pads_C2/TimeRes_Method_Direct.pdf}
%        \caption{No method}
%        \label{fig:TimeResMethod_Direct_HPKC2_160V}
%    \end{subfigure}
%    \begin{subfigure}{0.4\textwidth}
%        \centering
%        \includegraphics[width=\textwidth]{plots/HPK_pads_C2/TimeRes_Method_Weight2.pdf}
%        \caption{Weight squared method}
%        \label{fig:TimeResMethod_Weight2_HPKC2_160V}
%    \end{subfigure}
%    \caption{Time resolution of the HPK C2 pad detector with a Bias Voltage of 160 [V], using two different methods to obtain the detection time. Only the inner half of the detector is studied, demarcated by the red lines, to avoid edge effects.}
%    \label{fig:TimeResMethods_HPKC2}
%\end{figure}

%We use the simple maximum amplitude timestamp method to measure the time resolution as a function of the hit position for the HPK B2 and C2 sensors shown in Fig.~\ref{fig:TimeRes_HPKp}. The time resolution is about 30~ps and uniform across the sensor. 

%\begin{figure}
%    \centering
%    \includegraphics[width=0.49\textwidth]{plots/HPK_pads_C2/TimeRes_vs_x_weighted2_time_diff.pdf}
    %\label{fig:TimeRes_HPKC2p}
%    \includegraphics[width=0.49\textwidth]{plots/HPK_pads_B2/TimeRes_vs_x_weighted2_time_diff.pdf}
    %\label{fig:TimeRes_HPKB2p}
%    \caption{Time resolution of the pad detectors, using weight squared method vs tracker relative position, for nominal voltages. Only the inner half of the detector is studied, demarcated by the red lines, to avoid edge effects. \textcolor{red}{right-side x-axis for position, refer single/multi channel time resolutions instead of emphasizing weighted. Bigger font. Subtract tracker component.}
%    \textcolor{violet}{Is this plot needed? Maybe this info can be shown in the previous figure and remove this one.}}
%    \label{fig:TimeRes_HPKp}
%\end{figure}

In Fig.~\ref{fig:biasscanBNL}, we show the time and position resolution, averaged across the BNL2020 and BNL2021 sensors, as a function of the bias voltage. The time resolution improves from about 40~ps to 30~ps as the bias voltage is increased. The analogous measurement for the HPK B2 and C2 sensors are shown in Fig.~\ref{fig:biasscanHPK}, where we observe that the time resolution improves from XX~ps to YY~ps. 


\begin{figure}[htp]
\centering
\includegraphics[width=0.49\textwidth]{plots/resolution_plot_BNL2020}
\includegraphics[width=0.49\textwidth]{plots/resolution_plot_BNL2021_Medium}
\caption[Amp BNL 2020]{Time and position resolution as a function of bias voltage for the BNL 2020 (left) and BNL 2021 medium pitch (right) sensor. 
\label{fig:biasscanBNL}}
\end{figure}

\begin{figure}[htp]
\centering
\includegraphics[width=0.49\textwidth]{plots/HPK_pads_C2/resolution_plot_HPKC2.pdf}
%\includegraphics[width=0.49\textwidth]{plots/HPK_pads_B2/resolution_plot_HPKB2.pdf}
\caption[Amp HPK]{Time and position resolution as a function of bias voltage for the HPK C2 (left) and B2 (right) sensors. 
\label{fig:biasscanHPK}}
\end{figure}

